A simple backward construction of Branching Brownian motion with large displacement and applications

In this article, we study the extremal processes of branching Brownian motions conditioned on having an unusually large maximum. The limiting point measures form a one-parameter family and are the decoration point measures in the extremal processes of several branching processes, including branching Brownian motions with variable speed and multitype branching Brownian motions. We give a new, alternative representation of these point measures and we show that they form a continuous family. This also yields a simple probabilistic expression for the constant that appears in the large deviation probability of having a large displacement. As an application, we show that Bovier and Hartung (2015)'s results about variable speed branching Brownian motion also describe the extremal point process of branching Ornstein-Uhlenbeck processes.

==> fonctionC.tex <==
\begin{tikzpicture}[xscale=2,yscale=2.5]
  \draw[->] (-0.1,0) -- (5,0) node[below left] {$\rho$};
  \draw (1,0.033) -- (1,-0.033) node[below] {$1$};
  \draw[->] (0,-0.1) -- (0,1.3) node[left] {$C$};
  \draw (-0.1,1) node[left] {$\frac{1}{\sqrt{4\pi}}$} -- (0.1,1) ;
  \clip (0,0) rectangle (5,1.1);
  \draw[red] (1,0)--(2,4.183);
  \draw [dashed] (0.1,1) -- (10,1);
  \draw [thick, color=blue] (0.0,0) --(1.0,0.0) -- (1.01,0.109) -- (1.02,0.127) -- (1.03,0.146) -- (1.04,0.166) -- (1.05,0.185) -- (1.06,0.201) -- (1.07,0.219) -- (1.08,0.235) -- (1.09,0.251) -- (1.1,0.266) -- (1.11,0.28) -- (1.12,0.294) -- (1.13,0.307) -- (1.14,0.318) -- (1.15,0.33) -- (1.16,0.34) -- (1.17,0.351) -- (1.18,0.362) -- (1.19,0.372) -- (1.2,0.381) -- (1.21,0.391) -- (1.22,0.401) -- (1.23,0.41) -- (1.24,0.419) -- (1.25,0.428) -- (1.26,0.436) -- (1.27,0.443) -- (1.28,0.451) -- (1.29,0.458) -- (1.3,0.466) -- (1.31,0.473) -- (1.32,0.479) -- (1.33,0.486) -- (1.34,0.492) -- (1.35,0.498) -- (1.36,0.505) -- (1.37,0.512) -- (1.38,0.518) -- (1.39,0.524) -- (1.4,0.531) -- (1.41,0.537) -- (1.42,0.544) -- (1.43,0.549) -- (1.44,0.556) -- (1.45,0.562) -- (1.46,0.567) -- (1.47,0.572) -- (1.48,0.578) -- (1.49,0.583) -- (1.5,0.589) -- (1.51,0.594) -- (1.52,0.599) -- (1.53,0.604) -- (1.54,0.609) -- (1.55,0.614) -- (1.56,0.619) -- (1.57,0.623) -- (1.58,0.628) -- (1.59,0.632) -- (1.6,0.636) -- (1.61,0.641) -- (1.62,0.645) -- (1.63,0.649) -- (1.64,0.654) -- (1.65,0.658) -- (1.66,0.662) -- (1.67,0.666) -- (1.68,0.67) -- (1.69,0.673) -- (1.7,0.677) -- (1.71,0.681) -- (1.72,0.684) -- (1.73,0.688) -- (1.74,0.692) -- (1.75,0.695) -- (1.76,0.698) -- (1.77,0.701) -- (1.78,0.705) -- (1.79,0.708) -- (1.8,0.711) -- (1.81,0.714) -- (1.82,0.717) -- (1.83,0.72) -- (1.84,0.723) -- (1.85,0.726) -- (1.86,0.728) -- (1.87,0.731) -- (1.88,0.733) -- (1.89,0.736) -- (1.9,0.739) -- (1.91,0.741) -- (1.92,0.744) -- (1.93,0.746) -- (1.94,0.748) -- (1.95,0.751) -- (1.96,0.753) -- (1.97,0.755) -- (1.98,0.757) -- (1.99,0.76) -- (2.0,0.762) -- (2.01,0.765) -- (2.02,0.767) -- (2.03,0.769) -- (2.04,0.771) -- (2.05,0.773) -- (2.06,0.775) -- (2.07,0.777) -- (2.08,0.779) -- (2.09,0.781) -- (2.1,0.783) -- (2.11,0.785) -- (2.12,0.787) -- (2.13,0.789) -- (2.14,0.791) -- (2.15,0.793) -- (2.16,0.795) -- (2.17,0.796) -- (2.18,0.798) -- (2.19,0.8) -- (2.2,0.801) -- (2.21,0.802) -- (2.22,0.804) -- (2.23,0.806) -- (2.24,0.808) -- (2.25,0.81) -- (2.26,0.811) -- (2.27,0.813) -- (2.28,0.815) -- (2.29,0.817) -- (2.3,0.818) -- (2.31,0.82) -- (2.32,0.821) -- (2.33,0.822) -- (2.34,0.824) -- (2.35,0.825) -- (2.36,0.827) -- (2.37,0.828) -- (2.38,0.829) -- (2.39,0.83) -- (2.4,0.832) -- (2.41,0.833) -- (2.42,0.835) -- (2.43,0.836) -- (2.44,0.837) -- (2.45,0.839) -- (2.46,0.84) -- (2.47,0.841) -- (2.48,0.842) -- (2.49,0.843) -- (2.5,0.845) -- (2.51,0.846) -- (2.52,0.847) -- (2.53,0.848) -- (2.54,0.849) -- (2.55,0.851) -- (2.56,0.852) -- (2.57,0.853) -- (2.58,0.854) -- (2.59,0.855) -- (2.6,0.856) -- (2.61,0.857) -- (2.62,0.858) -- (2.63,0.86) -- (2.64,0.861) -- (2.65,0.862) -- (2.66,0.863) -- (2.67,0.864) -- (2.68,0.864) -- (2.69,0.865) -- (2.7,0.866) -- (2.71,0.867) -- (2.72,0.868) -- (2.73,0.869) -- (2.74,0.87) -- (2.75,0.871) -- (2.76,0.872) -- (2.77,0.873) -- (2.78,0.874) -- (2.79,0.874) -- (2.8,0.875) -- (2.81,0.876) -- (2.82,0.877) -- (2.83,0.878) -- (2.84,0.879) -- (2.85,0.88) -- (2.86,0.88) -- (2.87,0.881) -- (2.88,0.882) -- (2.89,0.883) -- (2.9,0.884) -- (2.91,0.884) -- (2.92,0.885) -- (2.93,0.886) -- (2.94,0.887) -- (2.95,0.887) -- (2.96,0.888) -- (2.97,0.889) -- (2.98,0.89) -- (2.99,0.89) -- (3.0,0.891) -- (3.01,0.892) -- (3.02,0.893) -- (3.03,0.893) -- (3.04,0.894) -- (3.05,0.894) -- (3.06,0.895) -- (3.07,0.896) -- (3.08,0.897) -- (3.09,0.897) -- (3.1,0.898) -- (3.11,0.898) -- (3.12,0.899) -- (3.13,0.9) -- (3.14,0.901) -- (3.15,0.901) -- (3.16,0.902) -- (3.17,0.903) -- (3.18,0.903) -- (3.19,0.904) -- (3.2,0.905) -- (3.21,0.905) -- (3.22,0.906) -- (3.23,0.906) -- (3.24,0.907) -- (3.25,0.908) -- (3.26,0.908) -- (3.27,0.909) -- (3.28,0.909) -- (3.29,0.91) -- (3.3,0.91) -- (3.31,0.911) -- (3.32,0.911) -- (3.33,0.912) -- (3.34,0.912) -- (3.35,0.913) -- (3.36,0.913) -- (3.37,0.914) -- (3.38,0.914) -- (3.39,0.915) -- (3.4,0.915) -- (3.41,0.916) -- (3.42,0.917) -- (3.43,0.917) -- (3.44,0.918) -- (3.45,0.918) -- (3.46,0.918) -- (3.47,0.919) -- (3.48,0.919) -- (3.49,0.92) -- (3.5,0.921) -- (3.51,0.921) -- (3.52,0.921) -- (3.53,0.922) -- (3.54,0.922) -- (3.55,0.923) -- (3.56,0.923) -- (3.57,0.924) -- (3.58,0.924) -- (3.59,0.924) -- (3.6,0.925) -- (3.61,0.925) -- (3.62,0.925) -- (3.63,0.926) -- (3.64,0.926) -- (3.65,0.927) -- (3.66,0.927) -- (3.67,0.928) -- (3.68,0.928) -- (3.69,0.928) -- (3.7,0.929) -- (3.71,0.929) -- (3.72,0.929) -- (3.73,0.93) -- (3.74,0.93) -- (3.75,0.93) -- (3.76,0.931) -- (3.77,0.931) -- (3.78,0.932) -- (3.79,0.932) -- (3.8,0.932) -- (3.81,0.933) -- (3.82,0.933) -- (3.83,0.933) -- (3.84,0.934) -- (3.85,0.934) -- (3.86,0.934) -- (3.87,0.935) -- (3.88,0.935) -- (3.89,0.935) -- (3.9,0.936) -- (3.91,0.936) -- (3.92,0.936) -- (3.93,0.937) -- (3.94,0.937) -- (3.95,0.938) -- (3.96,0.938) -- (3.97,0.938) -- (3.98,0.938) -- (3.99,0.939) -- (4.0,0.939) -- (4.01,0.939) -- (4.02,0.939) -- (4.03,0.94) -- (4.04,0.94) -- (4.05,0.94) -- (4.06,0.94) -- (4.07,0.941) -- (4.08,0.941) -- (4.09,0.941) -- (4.1,0.942) -- (4.11,0.942) -- (4.12,0.942) -- (4.13,0.942) -- (4.14,0.943) -- (4.15,0.943) -- (4.16,0.943) -- (4.17,0.944) -- (4.18,0.944) -- (4.19,0.944) -- (4.2,0.944) -- (4.21,0.945) -- (4.22,0.945) -- (4.23,0.945) -- (4.24,0.945) -- (4.25,0.946) -- (4.26,0.946) -- (4.27,0.946) -- (4.28,0.946) -- (4.29,0.947) -- (4.3,0.947) -- (4.31,0.947) -- (4.32,0.947) -- (4.33,0.948) -- (4.34,0.948) -- (4.35,0.948) -- (4.36,0.948) -- (4.37,0.949) -- (4.38,0.949) -- (4.39,0.949) -- (4.4,0.949) -- (4.41,0.949) -- (4.42,0.95) -- (4.43,0.95) -- (4.44,0.95) -- (4.45,0.951) -- (4.46,0.951) -- (4.47,0.951) -- (4.48,0.951) -- (4.49,0.951) -- (4.5,0.952) -- (4.51,0.952) -- (4.52,0.952) -- (4.53,0.952) -- (4.54,0.953) -- (4.55,0.953) -- (4.56,0.953) -- (4.57,0.953) -- (4.58,0.953) -- (4.59,0.954) -- (4.6,0.954) -- (4.61,0.954) -- (4.62,0.954) -- (4.63,0.954) -- (4.64,0.955) -- (4.65,0.955) -- (4.66,0.955) -- (4.67,0.955) -- (4.68,0.955) -- (4.69,0.955) -- (4.7,0.955) -- (4.71,0.956) -- (4.72,0.956) -- (4.73,0.956) -- (4.74,0.956) -- (4.75,0.956) -- (4.76,0.956) -- (4.77,0.957) -- (4.78,0.957) -- (4.79,0.957) -- (4.8,0.957) -- (4.81,0.957) -- (4.82,0.957) -- (4.83,0.957) -- (4.84,0.958) -- (4.85,0.958) -- (4.86,0.958) -- (4.87,0.958) -- (4.88,0.958) -- (4.89,0.958) -- (4.9,0.959) -- (4.91,0.959) -- (4.92,0.959) -- (4.93,0.959) -- (4.94,0.959) -- (4.95,0.959) -- (4.96,0.959) -- (4.97,0.96) -- (4.98,0.96) -- (4.99,0.96) -- (5.0,0.96) -- (5.01,0.96) -- (5.02,0.96) -- (5.03,0.961) -- (5.04,0.961) -- (5.05,0.961) -- (5.06,0.961) -- (5.07,0.961) -- (5.08,0.961) -- (5.09,0.962) -- (5.1,0.962) -- (5.11,0.962) -- (5.12,0.962) -- (5.13,0.962) -- (5.14,0.962) -- (5.15,0.962) -- (5.16,0.963) -- (5.17,0.963) -- (5.18,0.963) -- (5.19,0.963) -- (5.2,0.963) -- (5.21,0.963) -- (5.22,0.964) -- (5.23,0.964) -- (5.24,0.964) -- (5.25,0.964) -- (5.26,0.964) -- (5.27,0.964) -- (5.28,0.964) -- (5.29,0.964) -- (5.3,0.965) -- (5.31,0.965) -- (5.32,0.965) -- (5.33,0.965) -- (5.34,0.965) -- (5.35,0.965) -- (5.36,0.965) -- (5.37,0.965) -- (5.38,0.966) -- (5.39,0.966) -- (5.4,0.966) -- (5.41,0.966) -- (5.42,0.966) -- (5.43,0.966) -- (5.44,0.966) -- (5.45,0.966) -- (5.46,0.966) -- (5.47,0.967) -- (5.48,0.967) -- (5.49,0.967) -- (5.5,0.967) -- (5.51,0.967) -- (5.52,0.967) -- (5.53,0.967) -- (5.54,0.967) -- (5.55,0.968) -- (5.56,0.968) -- (5.57,0.968) -- (5.58,0.968) -- (5.59,0.968) -- (5.6,0.968) -- (5.61,0.968) -- (5.62,0.969) -- (5.63,0.969) -- (5.64,0.969) -- (5.65,0.969) -- (5.66,0.969) -- (5.67,0.969) -- (5.68,0.969) -- (5.69,0.969) -- (5.7,0.969) -- (5.71,0.97) -- (5.72,0.97) -- (5.73,0.97) -- (5.74,0.97) -- (5.75,0.97) -- (5.76,0.97) -- (5.77,0.97) -- (5.78,0.97) -- (5.79,0.97) -- (5.8,0.971) -- (5.81,0.971) -- (5.82,0.971) -- (5.83,0.971) -- (5.84,0.971) -- (5.85,0.971) -- (5.86,0.971) -- (5.87,0.971) -- (5.88,0.971) -- (5.89,0.971) -- (5.9,0.971) -- (5.91,0.971) -- (5.92,0.972) -- (5.93,0.972) -- (5.94,0.972) -- (5.95,0.972) -- (5.96,0.972) -- (5.97,0.972) -- (5.98,0.972) -- (5.99,0.972) -- (6.0,0.972) -- (6.01,0.972) -- (6.02,0.972) -- (6.03,0.972) -- (6.04,0.972) -- (6.05,0.973) -- (6.06,0.973) -- (6.07,0.973) -- (6.08,0.973) -- (6.09,0.973) -- (6.1,0.973) -- (6.11,0.973) -- (6.12,0.973) -- (6.13,0.973) -- (6.14,0.973) -- (6.15,0.974) -- (6.16,0.974) -- (6.17,0.974) -- (6.18,0.974) -- (6.19,0.974) -- (6.2,0.974) -- (6.21,0.974) -- (6.22,0.974) -- (6.23,0.974) -- (6.24,0.974) -- (6.25,0.974) -- (6.26,0.974) -- (6.27,0.974) -- (6.28,0.974) -- (6.29,0.974) -- (6.3,0.975) -- (6.31,0.975) -- (6.32,0.975) -- (6.33,0.975) -- (6.34,0.975) -- (6.35,0.975) -- (6.36,0.975) -- (6.37,0.975) -- (6.38,0.975) -- (6.39,0.975) -- (6.4,0.975) -- (6.41,0.976) -- (6.42,0.976) -- (6.43,0.976) -- (6.44,0.976) -- (6.45,0.976) -- (6.46,0.976) -- (6.47,0.976) -- (6.48,0.976) -- (6.49,0.976) -- (6.5,0.976) -- (6.51,0.976) -- (6.52,0.976) -- (6.53,0.977) -- (6.54,0.977) -- (6.55,0.977) -- (6.56,0.977) -- (6.57,0.977) -- (6.58,0.977) -- (6.59,0.977) -- (6.6,0.977) -- (6.61,0.977) -- (6.62,0.977) -- (6.63,0.977) -- (6.64,0.977) -- (6.65,0.977) -- (6.66,0.977) -- (6.67,0.977) -- (6.68,0.977) -- (6.69,0.978) -- (6.7,0.978) -- (6.71,0.978) -- (6.72,0.978) -- (6.73,0.978) -- (6.74,0.978) -- (6.75,0.978) -- (6.76,0.978) -- (6.77,0.978) -- (6.78,0.978) -- (6.79,0.978) -- (6.8,0.978) -- (6.81,0.978) -- (6.82,0.978) -- (6.83,0.978) -- (6.84,0.978) -- (6.85,0.979) -- (6.86,0.979) -- (6.87,0.979) -- (6.88,0.979) -- (6.89,0.979) -- (6.9,0.979) -- (6.91,0.979) -- (6.92,0.979) -- (6.93,0.979) -- (6.94,0.979) -- (6.95,0.979) -- (6.96,0.979) -- (6.97,0.979) -- (6.98,0.979) -- (6.99,0.979) -- (7.0,0.979) -- (7.01,0.98) -- (7.02,0.98) -- (7.03,0.98) -- (7.04,0.98) -- (7.05,0.98) -- (7.06,0.98) -- (7.07,0.98) -- (7.08,0.98) -- (7.09,0.98) -- (7.1,0.98) -- (7.11,0.98) -- (7.12,0.98) -- (7.13,0.98) -- (7.14,0.98) -- (7.15,0.98) -- (7.16,0.98) -- (7.17,0.98) -- (7.18,0.98) -- (7.19,0.98) -- (7.2,0.98) -- (7.21,0.98) -- (7.22,0.98) -- (7.23,0.981) -- (7.24,0.981) -- (7.25,0.981) -- (7.26,0.981) -- (7.27,0.981) -- (7.28,0.981) -- (7.29,0.981) -- (7.3,0.981) -- (7.31,0.981) -- (7.32,0.981) -- (7.33,0.981) -- (7.34,0.981) -- (7.35,0.981) -- (7.36,0.981) -- (7.37,0.981) -- (7.38,0.981) -- (7.39,0.981) -- (7.4,0.981) -- (7.41,0.981) -- (7.42,0.981) -- (7.43,0.981) -- (7.44,0.981) -- (7.45,0.981) -- (7.46,0.982) -- (7.47,0.982) -- (7.48,0.982) -- (7.49,0.982) -- (7.5,0.982) -- (7.51,0.982) -- (7.52,0.982) -- (7.53,0.982) -- (7.54,0.982) -- (7.55,0.982) -- (7.56,0.982) -- (7.57,0.982) -- (7.58,0.982) -- (7.59,0.982) -- (7.6,0.982) -- (7.61,0.982) -- (7.62,0.982) -- (7.63,0.982) -- (7.64,0.982) -- (7.65,0.982) -- (7.66,0.982) -- (7.67,0.982) -- (7.68,0.982) -- (7.69,0.983) -- (7.7,0.983) -- (7.71,0.983) -- (7.72,0.983) -- (7.73,0.983) -- (7.74,0.983) -- (7.75,0.983) -- (7.76,0.983) -- (7.77,0.983) -- (7.78,0.983) -- (7.79,0.983) -- (7.8,0.983) -- (7.81,0.983) -- (7.82,0.983) -- (7.83,0.983) -- (7.84,0.983) -- (7.85,0.983) -- (7.86,0.983) -- (7.87,0.983) -- (7.88,0.983) -- (7.89,0.983) -- (7.9,0.983) -- (7.91,0.983) -- (7.92,0.983) -- (7.93,0.983) -- (7.94,0.983) -- (7.95,0.983) -- (7.96,0.983) -- (7.97,0.984) -- (7.98,0.984) -- (7.99,0.984) -- (8.0,0.984) -- (8.01,0.984) -- (8.02,0.984) -- (8.03,0.984) -- (8.04,0.984) -- (8.05,0.984) -- (8.06,0.984) -- (8.07,0.984) -- (8.08,0.984) -- (8.09,0.984) -- (8.1,0.984) -- (8.11,0.984) -- (8.12,0.984) -- (8.13,0.984) -- (8.14,0.984) -- (8.15,0.984) -- (8.16,0.984) -- (8.17,0.984) -- (8.18,0.984) -- (8.19,0.984) -- (8.2,0.984) -- (8.21,0.984) -- (8.22,0.984) -- (8.23,0.984) -- (8.24,0.984) -- (8.25,0.984) -- (8.26,0.984) -- (8.27,0.984) -- (8.28,0.985) -- (8.29,0.985) -- (8.3,0.985) -- (8.31,0.985) -- (8.32,0.985) -- (8.33,0.985) -- (8.34,0.985) -- (8.35,0.985) -- (8.36,0.985) -- (8.37,0.985) -- (8.38,0.985) -- (8.39,0.985) -- (8.4,0.985) -- (8.41,0.985) -- (8.42,0.985) -- (8.43,0.985) -- (8.44,0.985) -- (8.45,0.985) -- (8.46,0.985) -- (8.47,0.985) -- (8.48,0.985) -- (8.49,0.985) -- (8.5,0.985) -- (8.51,0.985) -- (8.52,0.985) -- (8.53,0.986) -- (8.54,0.986) -- (8.55,0.986) -- (8.56,0.986) -- (8.57,0.986) -- (8.58,0.986) -- (8.59,0.986) -- (8.6,0.986) -- (8.61,0.986) -- (8.62,0.986) -- (8.63,0.986) -- (8.64,0.986) -- (8.65,0.986) -- (8.66,0.986) -- (8.67,0.986) -- (8.68,0.986) -- (8.69,0.986) -- (8.7,0.986) -- (8.71,0.986) -- (8.72,0.986) -- (8.73,0.986) -- (8.74,0.986) -- (8.75,0.986) -- (8.76,0.986) -- (8.77,0.986) -- (8.78,0.986) -- (8.79,0.986) -- (8.8,0.986) -- (8.81,0.986) -- (8.82,0.986) -- (8.83,0.986) -- (8.84,0.986) -- (8.85,0.986) -- (8.86,0.987) -- (8.87,0.987) -- (8.88,0.987) -- (8.89,0.987) -- (8.9,0.987) -- (8.91,0.987) -- (8.92,0.987) -- (8.93,0.987) -- (8.94,0.987) -- (8.95,0.987) -- (8.96,0.987) -- (8.97,0.987) -- (8.98,0.987) -- (8.99,0.987) -- (9.0,0.987) -- (9.01,0.987) -- (9.02,0.987) -- (9.03,0.987) -- (9.04,0.987) -- (9.05,0.987) -- (9.06,0.987) -- (9.07,0.987) -- (9.08,0.987) -- (9.09,0.987) -- (9.1,0.987) -- (9.11,0.987) -- (9.12,0.987) -- (9.13,0.987) -- (9.14,0.987) -- (9.15,0.987) -- (9.16,0.987) -- (9.17,0.987) -- (9.18,0.987) -- (9.19,0.988) -- (9.2,0.988) -- (9.21,0.988) -- (9.22,0.988) -- (9.23,0.988) -- (9.24,0.988) -- (9.25,0.988) -- (9.26,0.988) -- (9.27,0.988) -- (9.28,0.988) -- (9.29,0.988) -- (9.3,0.988) -- (9.31,0.988) -- (9.32,0.988) -- (9.33,0.988) -- (9.34,0.988) -- (9.35,0.988) -- (9.36,0.988) -- (9.37,0.988) -- (9.38,0.988) -- (9.39,0.988) -- (9.4,0.988) -- (9.41,0.988) -- (9.42,0.988) -- (9.43,0.988) -- (9.44,0.988) -- (9.45,0.988) -- (9.46,0.988) -- (9.47,0.988) -- (9.48,0.988) -- (9.49,0.988) -- (9.5,0.988) -- (9.51,0.988) -- (9.52,0.988) -- (9.53,0.988) -- (9.54,0.988) -- (9.55,0.988) -- (9.56,0.988) -- (9.57,0.988) -- (9.58,0.988) -- (9.59,0.988) -- (9.6,0.988) -- (9.61,0.988) -- (9.62,0.988) -- (9.63,0.988) -- (9.64,0.988) -- (9.65,0.988) -- (9.66,0.988) -- (9.67,0.988) -- (9.68,0.989) -- (9.69,0.989) -- (9.7,0.989) -- (9.71,0.989) -- (9.72,0.989) -- (9.73,0.989) -- (9.74,0.989) -- (9.75,0.989) -- (9.76,0.989) -- (9.77,0.989) -- (9.78,0.989) -- (9.79,0.989) -- (9.8,0.989) -- (9.81,0.989) -- (9.82,0.989) -- (9.83,0.989) -- (9.84,0.989) -- (9.85,0.989) -- (9.86,0.989) -- (9.87,0.989) -- (9.88,0.989) -- (9.89,0.989) -- (9.9,0.989) -- (9.91,0.989) -- (9.92,0.989) -- (9.93,0.989) -- (9.94,0.989) -- (9.95,0.989) -- (9.96,0.989) -- (9.97,0.989) -- (9.98,0.989) -- (9.99,0.989);
\end{tikzpicture}

